Towards a general framework for improving the performance of classifiers using XAI methods

Modern Artificial Intelligence (AI) systems, especially Deep Learning (DL) models, poses challenges in understanding their inner workings by AI researchers. eXplainable Artificial Intelligence (XAI) inspects internal mechanisms of AI models providing explanations about their decisions. While current XAI research predominantly concentrates on explaining AI systems, there is a growing interest in using XAI techniques to automatically improve the performance of AI systems themselves. This paper proposes a general framework for automatically improving the performance of pre-trained DL classifiers using XAI methods, avoiding the computational overhead associated with retraining complex models from scratch. In particular, we outline the possibility of two different learning strategies for implementing this architecture, which we will call auto-encoder-based and encoder-decoder-based, and discuss their key aspects.

==> _discussion.tex <==
\input{_FIG_XAI}

\section{Discussion}
\label{sec:discussion}

In \Cref{fig:imagesXAItoImprove_CIFAR10,fig:imagesXAItoImprove_CIFAR100,fig:imagesXAItoImprove_STL10}, images from the CIFAR-10, CIFAR-100, and STL-10 test sets are presented, illustrating instances where the IMPACTX method successfully corrects the classification made by the LeNet-5 model as baseline. For each input image is shown: the explanation corresponding to the class predicted by $M$ (baseline), denoted as $\vec{r_{M(\vec{x})}}\in SHAP(M, \vec{x})$, and the explanation reconstructed through the Encoder-Decoder $LEP-D(\vec{x})$ of the IMPACTX architecture, using LeNet-5 as architecture for the $LEP$ encoder. For each image, the class and score given by baseline model and the IMPACTX approach are provided. 

It's evident that in the majority of cases, the reconstructed explanations focus on input regions that are intuitively more relevant to the true output compared to the explanation corresponding to the $M$ response. Thus, highlighting the effectiveness of IMPACTX in generating knowledge useful for the correct prediction.
For example, in \cref{fig:imagesXAItoImprove_CIFAR100}, the effectiveness of IMPACTX in accurately classifying a tiger is clearly visible, in contrast to the baseline which had mistakenly identified the animal as a leopard. Similarly, IMPACTX allows to correctly classify a leopard. The explanations provided by IMPACTX are remarkably clear, highlighting distinctive characteristic elements of the two animals. This includes the bright orange fur with vertical black stripes typical of tigers, and the golden-yellow coat with black spots, known as rosettes, distinctive of leopards.
In \cref{fig:imagesXAItoImprove_STL10}, we observe some instances where the baseline model incorrectly identifies an airplane as a bird, whereas IMPACTX classifies correctly these images as airplanes, also highlighting the distinctive elements of an airplanes.
Again, in \cref{fig:imagesXAItoImprove_CIFAR10}, IMPACTX corrects the baseline classification. Moreover explanations seem particularly significant in the classes of cats, trucks, and airplanes.

\begin{figure*}[h!]
\centering
%% 1
    \begin{subfigure}[t]{0.43\linewidth}
    \centering
    \includegraphics[width=1\textwidth]{FIG/confusionMatrix_stl10_MobilNet_baseline.png}
    \caption{Baseline, accuracy: 91.07 }
    \label{fig:cm_baseline}
    \end{subfigure}\hfill
%% 2
    \begin{subfigure}[t]{0.5\linewidth}
    %\centering\vspace{-7em}
    \includegraphics[width=1\textwidth]{FIG/confusionMatrix_stl10_MobilNet_proposal.png} 
    %vspace{2.8em}
    \caption{IMPACTX, accuracy: 95.79}
    \label{fig:cm_proposal}
    \end{subfigure}\hfill  
\caption{Confusion matrices for the STL-10 test set, using MobileNet as baseline (a) and with the proposed method IMPACTX (b). The main diagonal in (b) illustrates that the enhancements introduced by our approach are evenly distributed across all classes, highlighting the positive impact of the proposed method on the model's performance across a diverse range of categories.} 
\label{fig:cm}
\end{figure*}

To better understand whether the improvements achieved by our approach were specific to a few classes or distributed across all classes, we also computed the confusion matrices for MobileNet (baseline) and the IMPACTX approach on the STL-10 test set (see \cref{fig:cm}). 
From the confusion matrices, one can note that the improvements introduced by our approach are uniformly distributed across all classes of the inspected dataset. This observation underlines the positive and comprehensive impact of the proposed method in improving the performance of the model across a wide range of categories.
